LLM-Based Invariant Testing for Software Functional Bugs

Manually writing unit tests to uncover functional bugs in software libraries is not only time-consuming but also requires a deep understanding of the intended semantics of the APIs. Heuristic-based test generation methods suffer from low usability because they cannot reason about program semantics or interpret source code and documentation as humans do. Traditional fuzzing techniques like OSS-Fuzz often rely on crashes to detect bugs, but functional bugs do not always cause crashes. To overcome these limitations, we present LISA, a novel LLM-based invariant testing framework for software functional bugs. LISA iteratively generates API sequences and program invariants guided by API n-gram feedback, achieving higher bug-detection rates and competitive code coverage compared with both fuzzing and prior LLM-based test generation approaches, and reporting each finding as a high-confidence bug candidate for developer confirmation.

==> code/bug_code.tex <==
\begin{lstlisting} [
    language=C++, 
    caption={Example of functional bug injection}, 
    label=lst:bug_code,
    frame=single,
]
// original code
int read_employee_count(Store *store) {
    return store->employee_count;
}

// code with functional bug (introduces a hidden mutation)
int read_employee_count(Store *store) {
    store->customer_count++;   // unintended side-effect: converts read into write
    return store->employee_count;
}
\end{lstlisting}

